Automatic Scoring of Dream Reports' Emotional Content with Large Language Models

In the field of dream research, the study of dream content typically relies on the analysis of verbal reports provided by dreamers upon awakening from their sleep. This task is classically performed through manual scoring provided by trained annotators, at a great time expense. While a consistent body of work suggests that natural language processing (NLP) tools can support the automatic analysis of dream reports, proposed methods lacked the ability to reason over a report's full context and required extensive data pre-processing. Furthermore, in most cases, these methods were not validated against standard manual scoring approaches. In this work, we address these limitations by adopting large language models (LLMs) to study and replicate the manual annotation of dream reports, using a mixture of off-the-shelf and bespoke approaches, with a focus on references to reports' emotions. Our results show that the off-the-shelf method achieves a low performance probably in light of inherent linguistic differences between reports collected in different (groups of) individuals. On the other hand, the proposed bespoke text classification method achieves a high performance, which is robust against potential biases. Overall, these observations indicate that our approach could find application in the analysis of large dream datasets and may favour reproducibility and comparability of results across studies.

==> _images/USA_dremaer_box.tex <==

\begin{figure}[htb!]
    \centering
    \includegraphics[width=\columnwidth]{_images/USA_one_emotion_bar.png}
    \caption{\label{fig:emotion_cluster_box} Emotion alignment results. Percentage of one-emotion reports classified by the model as \texttt{POSITIVE}. Variance is generated by results from different Dream Bank's collections and emotion sets (dreamer vs. general).}
\end{figure}  


==> _images/dreambank_example.tex <==


\begin{figure}[tbhp]
\centering
\includegraphics[width=\linewidth]{_images/dreambank_example_Bea.pdf}
\caption{Example of a dream report from Dream Bank, with its annotation according to the Hall and Van de Castle (HVDC) scoring system. In this work, we focus on the Emotions set feature.}
\label{fig:scoring_example}
\end{figure}

==> _images/textclass_collections_dreamer.tex <==

\begin{figure}[htb!]
    \centering
    \includegraphics[width=\columnwidth]{_images/textclass_collections_dreamer.png}
    \caption{\label{fig:textclass_coll_dreamer}Text classification ablation results. F1 Weighted average scores obtained by the model when each Dream Bank Series is held out of training and used as test set. The dashed vertical line reports the average F1 Weighted average obtained in the main experiment (see Table \ref{tab:multi_class_kfold_overall}). }
\end{figure}  

==> _images/textclass_collections_overall.tex <==



% \begin{figure*}[htb!]
%     \centering
%     \includegraphics[width=\columnwidth]
%      \begin{subfigure}[b]{0.5\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{_images/textclass_collections_dreamer.png}
%          \caption{$y=x$}
%          \label{fig:y equals x}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.5\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{_images/textclass_collections_general.png}
%          \caption{$y=3\sin x$}
%          \label{fig:three sin x}
%      \end{subfigure}
%      \hfill
% \end{figure*}


\begin{figure*}
     \centering
     \begin{subfigure}[a]{\columnwidth}
         \centering
         \includegraphics[width=.4\columnwidth]{_images/textclass_collections_general.png}
         \caption{General}
         \label{fig:ablation_general}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{\columnwidth}
         \centering
         \includegraphics[width=.4\columnwidth]{_images/textclass_collections_dreamer.png}
         \caption{Dreamer}
         \label{fig:ablation_dreamer}
     \end{subfigure}
     \hfill
        \caption{Ablation results. F1 Weighted average scores obtained by the model when each Dream Bank's Series was held out from training and used solely as test set. The dashed vertical lines reports the average F1 Weighted  obtained in the main experiment (see Table \ref{tab:multi_class_kfold_overall}).}
        \label{fig:textclass_coll_all}
\end{figure*}

==> _tables/text_class_dreamer.tex <==

% \begin{table}[htb!]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{rcccc}
% \hlineB{3}
%   & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} & \textbf{Support} \\
% \hlineB{3}
% Anger   (AN)         & .872               & .860            & .860              & 31.4             \\
% Apprehension   (AP)  & .878               & .870            & .874              & 75.0             \\
% Confusion   (CO)     & .900               & .786            & .836              & 33.6             \\
% Sadness   (SA)       & .862               & .798            & .828              & 24.6             \\
% Happiness   (HA)     & .868               & .878            & .872              & 36.0             \\
% \hline
% Micro   average         & .876               & .850            & .858              & 20.6             \\
% Macro   average         & .876               & .838            & .852              & 20.6             \\
% Weighted   average      & .878               & .850            & .858              & 20.6             \\
% Samples   average       & .890               & .880            & .872              & 20.6    \\
% \hlineB{3}
% \end{tabular}
% }
% \caption{\label{fig:multi_class_kfold} Text classification results. Overall results for the multi-label supervised text classification experiment. Scores report average (± standard deviation).}
% \end{table}



\begin{table}[htb!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{rccc}
\hlineB{3}
  & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\
\hlineB{3}
Anger   (AN)         & 87 ± 6                   & 86 ± 6            & 86 ± 1  \\
Apprehension   (AP)  & 87 ± 3                   & 87 ± 6            & 87 ± 3  \\
Confusion   (CO)     & 90 ± 5                   & 78 ± 3            & 83 ± 3 \\
Sadness   (SD)       & 86 ± 2                   & 79 ± 7            & 82 ± 4  \\
Happiness   (HA)     & 86 ± 3                   & 87 ± 7            & 87 ± 4 \\
\hline
Micro   avg.         & 87 ± 2               & 85 ± 3            & 85 ± 2 \\
Macro   avg.         & 87 ± 2               & 83 ± 3            & 85 ± 2  \\
Weighted   avg.      & 87 ± 2               & 85 ± 3            & 85 ± 2   \\
Samples   avg.       & 89 ± 3               & 88 ± 3            & 87 ± 2  \\
\hlineB{3}
\end{tabular}
}
\caption{\label{tab:multi_class_kfold} Text classification results: Dreamer emotion. Overall results for the multi-label supervised text classification experiment. Scores report the five-fold average (± standard deviation).}
\end{table}

==> _tables/text_class_general.tex <==

% \begin{table}[htb!]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{rcccc}
% \hlineB{3}
%   & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} & \textbf{Support} \\
% \hlineB{3}
% Anger   (AN)         & .872               & .860            & .860              & 31.4             \\
% Apprehension   (AP)  & .878               & .870            & .874              & 75.0             \\
% Confusion   (CO)     & .900               & .786            & .836              & 33.6             \\
% Sadness   (SA)       & .862               & .798            & .828              & 24.6             \\
% Happiness   (HA)     & .868               & .878            & .872              & 36.0             \\
% \hline
% Micro   average         & .876               & .850            & .858              & 20.6             \\
% Macro   average         & .876               & .838            & .852              & 20.6             \\
% Weighted   average      & .878               & .850            & .858              & 20.6             \\
% Samples   average       & .890               & .880            & .872              & 20.6    \\
% \hlineB{3}
% \end{tabular}
% }
% \caption{\label{fig:multi_class_kfold} Text classification results. Overall results for the multi-label supervised text classification experiment. Scores report average (± standard deviation).}
% \end{table}



\begin{table}[htb!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{rccc}
\hlineB{3}
  & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\
\hlineB{3}
Anger (AN)        & 81 ± 4        & 91 ± 3        & 86 ± 3 \\
Apprehension (AP) & 88 ± 3        & 94 ± 3        & 91 ± 2 \\
Sadness (SD)      & 78 ± 8        & 87 ± 2        & 82 ± 6 \\
Confusion (CO)    & 90 ± 4        & 88 ± 5        & 89 ± 4 \\
Happyness (HA)    & 86 ± 5        & 88 ± 4        & 87 ± 2 \\ \hline
Micro avg.        & 85 ± 2        & 90 ± 2        & 88 ± 1 \\
Macro avg.        & 85 ± 2        & 89 ± 1        & 87 ± 2 \\
Weighted avg.     & 86 ± 1        & 90 ± 2        & 88 ± 1 \\
Samples avg.      & 88 ± 1        & 91 ± 2        & 88 ± 1 \\ \hline
\hlineB{3}
\end{tabular}
}
\caption{\label{tab:multi_class_kfold_gen} Text classification results: General emotion. Overall results for the multi-label supervised text classification experiment. Scores report the five-fold average (± standard deviation).}
\end{table}

==> _tables/text_class_overall.tex <==


\begin{table*}[htb!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{rcccccc}
\hlineB{3}
                     & \multicolumn{2}{c}{\textbf{Precision}} & \multicolumn{2}{c}{\textbf{Recall}} & \multicolumn{2}{c}{\textbf{F1}} \\
\multicolumn{1}{l}{} & General       & Dreamer       & General      & Dreamer     & General    & Dreamer   \\ \hlineB{3}
Anger (AN)           & 81 ± 4        & 87 ± 6        & 91 ± 3       & 86 ± 6      & 86 ± 3     & 86 ± 1    \\
Apprehension (AP)    & 88 ± 3        & 87 ± 3        & 94 ± 3       & 87 ± 6      & 91 ± 2     & 87 ± 3    \\
Sadness (SD)         & 78 ± 8        & 90 ± 5        & 87 ± 2       & 78 ± 3      & 82 ± 6     & 83 ± 3    \\
Confusion (CO)       & 90 ± 4        & 86 ± 2        & 88 ± 5       & 79 ± 7      & 89 ± 4     & 82 ± 4    \\
Happyness (HA)       & 86 ± 5        & 86 ± 3        & 88 ± 4       & 87 ± 7      & 87 ± 2     & 87 ± 4    \\ \hline
Micro avg.           & 85 ± 2        & 87 ± 2        & 90 ± 2       & 85 ± 3      & 88 ± 1     & 85 ± 2    \\
Macro avg.           & 85 ± 2        & 87 ± 2        & 89 ± 1       & 83 ± 3      & 87 ± 2     & 85 ± 2    \\
Weighted avg.        & 86 ± 1        & 87 ± 3        & 90 ± 2       & 85 ± 3      & 88 ± 1     & 85 ± 2    \\
Samples avg.         & 88 ± 1        & 89 ± 3        & 91 ± 2       & 88 ± 3      & 88 ± 1     & 87 ± 2    \\ \hlineB{3}
\end{tabular}
}
\caption{\label{tab:multi_class_kfold_overall} Text classification results. Average scores (± standard deviation) of the 5-fold cross-validation supervised experiment based on emotion presence.}
\end{table*}

